Diffusion-NAT: Self-Prompting Discrete Diffusion for Non-Autoregressive Text Generation

Recently, continuous diffusion models (CDM) have been introduced into non-autoregressive (NAR) text-to-text generation. However, the discrete nature of text increases the difficulty of CDM to generate coherent and fluent texts, and also causes the incompatibility problem between CDM and advanced NLP techniques, especially the popular pre-trained language models~(PLMs). To solve it, we propose Diffusion-NAT, which introduces discrete diffusion models~(DDM) into NAR text-to-text generation and integrates BART to improve the performance. By revising the decoding process of BART and the typical settings of DDM, we unify the inference process of BART and the denoising process of DDM into the same NAR masked tokens recovering task. In this way, DDM can rely on BART to perform denoising, which can benefit from both the rich pre-learned knowledge of BART and the iterative refining paradigm of DDM. Besides, we also propose the iterative self-prompting strategy to further improve the generation quality. Experimental results on 7 datasets show that our approach can outperform competitive NAR methods, and even surpass autoregressive methods. Our code and data will be publicly released.

==> model.tex <==
\section{Approach}
Our proposed Diffusion-NAT focuses on adapting PLMs into discrete diffusion models for effective NAR text-to-text generation.
In our approach, we leverage a Seq2Seq PLM, BART~\cite{DBLP:conf/acl/LewisLGGMLSZ20} as the backbone, and unify its inference process and the denoising process of discrete diffusion models into the masked tokens recovering task in a NAR manner.
Based on it, we also adjust the detailed settings of the PLM and typical discrete diffusion models, \eg removing time step embeddings, to further reduce their divergence for better adaptation.
Besides, we also propose the iterative self-prompting strategy that allows the PLM to deliberate and improve the intermediately generated texts during inference. 
The overview of our approach is shown in Figure~\ref{}.

\subsection{Adjusting the PLM for NAR Masked Tokens Recovering}
Most generative PLMs~\cite{radford2019language,DBLP:conf/acl/LewisLGGMLSZ20} rely on the token-by-token autoregressive paradigm for decoding.
Such a way is inconsistent with the NAR text generation task and would be unaffordable if combining with the iterative denoising process of diffusion models.
%Seq2Seq PLM, \eg BART~\cite{} and T5~\cite{}, have been pre-trained on large-scale corpus with generation-related tasks, and have shown superiority in a variety of text generation tasks.
Therefore, we aim to adjust it as the masked tokens recovering process in a NAR manner, which is similar to the pre-training task of the PLM and can better align with the discrete diffusion models.


\paragraph{The Seq2Seq PLM BART.}
BART~\cite{DBLP:conf/acl/LewisLGGMLSZ20} is a Seq2Seq PLM that has been widely-used on various text-to-text generation tasks.
It incorporates the encoder-decoder Transformer architecture.
Given the input text $C$, the encoder produces its representation vectors $\mathbf{E}$, and the decoder performs cross-attention with $\mathbf{E}$ to inject the condition from the input text.
During pre-training, the denoising autoencoding task is adopted to learn the model parameters on a large-scale corpus, which focuses on recovering the corrupted text (\eg part of tokens are replaced by ``$\texttt{[MASK]}$'').
%Given the input text $C$, BART incorporates the bidirectional Transformer encoder to aggregate the useful information for each token, and produce the input representation vectors $\mathbf{E}$.
During inference, using a start token as the initial input of the decoder, the output text will be generated token by token.
%In this way, the cross-attention with $\mathbf{E}$ are performed to inject the condition from the input text.
%Concretely, a certain percent of tokens from the input text will be randomly selected for masking (\ie replaced by the token ``$\texttt{[MASK]}$''), and PLMs are trained to accurately recover them.

\paragraph{Revising Decoding Process.} \label{sec-decoding}
To unify the inference and denoising processes of the PLM and diffusion model, it is essential to convert the AR generation paradigm of BART into the masked tokens recovering process in a NAR fashion.
Therefore, the key is to revise the decoding process of BART to support recovering all masked tokens simultaneously.
Concretely, we first revise the initial input of the decoder from the start token into a sequence of $\texttt{[MASK]}$ tokens.
Then, BART requires to rely on the conditions from the encoder to simultaneously recover all the $\texttt{[MASK]}$ tokens into the output text, denoted as:
\begin{equation}
    \text{PLM}(\{[\texttt{M}], \cdots, [\texttt{M}]\}, \mathcal{C})=\{y_{1}, \cdots, y_{n}\},
\end{equation}
where $\texttt{[M]}$ denotes the $\texttt{[MASK]}$ token. 
In this way, the decoding process would be the NAR masked tokens recovering task.
As it is similar to the pre-training task of BART, such a way can effectively reuse the learned knowledge during pre-training for NAR text generation.
%we can also leverage Eq.~\ref{eq-CE} to fine-tune the model parameters.

\subsection{Discrete Diffusion Models using the PLM for NAR Masked Tokens Recovering}
Given the condition $\mathcal{C}$ and a sequence of $\texttt{[MASK]}$ tokens, we utilize the discrete diffusion process to generate the output text.
To better combine it with the PLM, we adjust the typical settings of discrete diffusion models, including the Markov transition matrices, time step embeddings, and the training objective.

\paragraph{Markov Transition Matrices with $\texttt{[MASK]}$.}
As introduced in Section~\ref{sec-problem}, discrete diffusion models rely on the probability transition matrix $\mathbf{Q}_{t}$ to perform the forward and denoising processes.
To convert the denoising process in each step into the masked tokens recovering task, we adopt the transition matrix with the absorbing state $\texttt{[MASK]}$.
Concretely, at the $t$-th step of the forward process, if the token $i$ is not the $\texttt{[MASK]}$ token, it has the probabilities $\alpha_t$ and $\gamma_t$ to be unchanged and replaced by the $\texttt{[MASK]}$ token respectively, leaving the probability of $\beta_t=1-\alpha_t-\gamma_t$ transiting to other tokens in $\mathcal{V}$ as:
\begin{equation}
    [\mathbf{Q}_{t}]_{i,j}=\left\{
\begin{aligned}
&\alpha_{t},& &\text{if} \   j=i,& \\
&\gamma_{t},& &\text{if} \   j=\texttt{[M]},& \\
&1-\alpha_t-\gamma_t,& &\text{otherwise},&
\end{aligned}
\right.
\end{equation}
where $\alpha_t$ and $\gamma_t$ are determined by the pre-defined noise schedule, \eg cosine~\cite{DBLP:conf/icml/NicholD21} and spindle~\cite{DBLP:journals/corr/abs-2211-15029}.
If the token is the $\texttt{[MASK]}$ token, it will be unchanged. 
Based on such forward process, all tokens from the output text would become $\texttt{[MASK]}$ after a sufficient number of steps, corresponding to the all-$\texttt{[MASK]}$ initial input of the decoder.
In the denoising process, we incorporate the PLM to gradually recover the all-$\texttt{[MASK]}$ sequence into output text in the NAR manner.
In this way, each denoising step is equivalent to the decoding of the PLM in Section~\ref{sec-decoding}, unifying the objective of both.

\paragraph{Removing Time Step Embeddings.}
As introduced in Section~\ref{sec-problem}, typical diffusion models require the time step embeddings to represent the time information~\cite{DBLP:conf/nips/HoJA20,DBLP:conf/iclr/SongME21}.
Generally, the time step embeddings will be feed into the U-Net or Transformer model and are added into the embeddings or hidden states.
However, as PLMs have never seen time step embeddings during pre-training, the above way would affect the latent space of PLMs and increase the computational and training burden.
Actually, as the discrete diffusion process is to progressively recover the all-$\texttt{[MASK]}$ sequence, the PLM can directly acquire the time information by counting the number of $\texttt{[MASK]}$ tokens.
Therefore, we remove the time step embeddings in our approach.
In this way, we can directly reuse the architecture and pre-trained parameters of the PLM.
Furthermore, as such a way allows PLMs to ignore the current time step during performing iterative denoising, it also better suits the commonly-used DDIM method~\cite{DBLP:conf/iclr/SongME21} that incorporates the non-Markov process for the fast inference of diffusion models.


\paragraph{Training with NAR Masked Tokens Recovering.}
During training, existing diffusion models mostly learn to predict the noise in the current time step.
However, such training objective is not consistent with PLMs.
% and it is hard to directly predict the noise in the discrete diffusion process.
Inspired by existing works~\cite{DBLP:journals/corr/abs-2205-14217,DBLP:journals/corr/abs-2210-08933}, we aim to predict the original text tokens $Y_0=\{y^{(0)}_1, \cdots, y^{(0)}_n\}$ in the NAR manner at each time step.
The training objective is formulated as:
\begin{equation}
    \mathcal{L}_{Y}=%-\log p_{\theta}(Y_0|Y_t, C)=
    -\sum_{i=1}^{n}\log p_{\theta}(y^{(0)}_i|Y_t, C)
    \label{eq-mlm}
\end{equation}
where $Y_t$ denotes the intermediate recovered text in the $t$-th step.
As $Y_t$ commonly contains several $\texttt{[MASK]}$ tokens, the above training objective can be regarded as learning to recover these masked tokens.
Such a training objective is similar to the pre-training objective of BART, helping it adapt better for the diffusion process.
During inference, given $Y_t$, our model also first estimates $\hat{Y}_0$, and then adds the $\{t-1\}$-step noise into it for producing $Y_{t-1}$.
The above process would iterate for multiple steps, until obtaining the final results of $Y_0$.

\subsection{Iterative Self-Prompting}
In the typical denoising process, the denoising network relies on the condition $C$ and $Y_t$ to estimate $\hat{Y}_0$.
However, in early steps, $\texttt{[MASK]}$ tokens generally occupy the majority of $Y_t$, causing the estimation much difficult.
Motivated by the self-conditioning strategy~\cite{DBLP:journals/corr/abs-2208-04202}, we propose the iterative self-prompting strategy that endows our model the deliberation capacity via prefixed prompts, to reduce the estimation difficulty during inference.

\paragraph{Training with Self-Prompting.}
%As introduced before, we utilize PLMs to predict the original tokens $\hat{Y}_0$ based on $Y_t$ and $C$ in each step.
Our proposed self-prompting strategy focuses on improving the quality of $\hat{Y}_0$ through multi-round checking and revision.
To achieve it, we construct the prompt using the generated results from the PLM, and then prefix it with the condition $C$ to feed the PLM in many times.
Concretely, given $Y_t$ and $C$, we first utilize the PLM to produce the estimated $\hat{Y}_0$.
Then, as $\hat{Y}_0$ and $C$ are two sequences of tokens, we regard $\hat{Y}_0$ as the prompt of the PLM and prefix it with $C$ to compose the new input condition $C'=[\hat{Y}_0;C]$.
Next, the new condition $C'$ and $Y_t$ are fed into the encoder and decoder of the PLM respectively, where the cross-attention in the decoder would help the PLM produce more high-quality $\hat{Y}'_0$ with the consideration of the previous one.
During training, with a certain probability (\eg 50\%), we do not use the self-prompting strategy and only optimize the model parameter using Eq.~\ref{eq-mlm}.
At other times, we first produce $\hat{Y}_0$ and then construct $C'$ for self-prompting, where the training objective becomes:
\begin{equation}
    \mathcal{L}_{Y}=-\sum_{i=1}^{n}\log p_{\theta}(y^{(0)}_i|Y_t, \hat{Y}_0, C)%-\log p_{\theta}(Y_0|Y_t, \hat{Y}_0, C).
\end{equation}

\paragraph{Inference with Iterative Self-Prompting.}
As the above training process has endowed our model the capacity of using the conditions from the previous estimated $\hat{Y}_0$, we can iterate such a self-prompting process in many times during inference, until obtain a well-estimated $\hat{Y}_0$.
Specifically, we repeat the process for $K$ times that first estimates the original tokens $\hat{Y}_0$ based on the constructed new condition $C'$ and then utilizes it to replace the original prompt within $C'$.
In this way, by setting proper hyper-parameter $K$, we can balance the accuracy of the estimated $\hat{Y}_0$ and the time cost during inference.
Note that such a way also supports adding explicit controls in the intermediate prompts for guiding the generation, \eg correcting the grammar errors in $\hat{Y}_0$.
We leave it into our future work.

